Robosourcing Educational Resources -- Leveraging Large Language Models for Learnersourcing

In this article, we introduce and evaluate the concept of robosourcing for creating educational content. Robosourcing lies in the intersection of crowdsourcing and large language models, where instead of a crowd of humans, requests to large language models replace some of the work traditionally performed by the crowd. Robosourcing includes a human-in-the-loop to provide priming (input) as well as to evaluate and potentially adjust the generated artefacts; these evaluations could also be used to improve the large language models. We propose a system to outline the robosourcing process. We further study the feasibility of robosourcing in the context of education by conducting an evaluation of robosourced and programming exercises, generated using OpenAI Codex. Our results suggest that robosourcing could significantly reduce human effort in creating diverse educational content while maintaining quality similar to human-created content.

==> 00-abstract.tex <==

In this article, we introduce and evaluate the concept of robosourcing for creating educational content. Robosourcing lies in the intersection of crowdsourcing and large language models, where instead of a crowd of humans, requests to large language models 
%are used as the crowd. 
replace some of the work traditionally performed by the crowd.
Robosourcing includes a human-in-the-loop to provide priming (input) as well as to evaluate and potentially adjust the generated artefacts; these evaluations could also be used to improve the large language models. We propose a system to outline the robosourcing process. We further study the feasibility of robosourcing in the context of education by conducting an evaluation of robosourced and programming exercises, generated using OpenAI Codex. Our results suggest that robosourcing could significantly reduce human effort in creating diverse educational content while maintaining quality similar to human-created content.

==> 20-background.tex <==

\section{Background}

\subsection{Drill and practice}

Across a wide range of educational contexts, drill and practice activities are both popular and highly effective.  In a review of the efficacy of commonly used learning strategies, Dunlosky rated ``practice testing'', particularly when
repeated over multiple study sessions, as the most effective technique for enhancing learning and boosting student achievement \cite{dunlosky2013strengthening}.  The benefits of drill and practice style testing are widely known, generating headlines in popular media.  For example, a 2011 article in the New York Times entitled ``To Really Learn, Quit Studying and Take a Test''\footnote{https://www.nytimes.com/2011/01/21/science/21memory.html} espoused the unique benefits of being tested when compared with several other common study techniques.  These benefits are underpinned by a robust phenomenon known as the \emph{testing effect}, which posits that being tested on previously studied material is more beneficial with respect to long-term retention of the material than multiple episodes of studying \cite{Roediger_2013_RPT}.  This effect has been well established both in controlled laboratory environments and in the classroom.  A meta-review of the testing effect in classroom environments shows clear evidence that frequent testing yields positive effects on both perceived and actual learning outcomes \cite{Bangert_1991_FCT}.

The primary challenge of supporting drill and practice activities at scale is the human effort associated with generating questions and associated solutions.  Practice exercises should ideally be personalized to the needs of individual learners, and thus large repositories that cover all relevant concepts are required \cite{ericsson2018cambridge}.  In addition, research on the problem description effect has shown that the presence of relevant contextual information in the natural language wording of a question can impact cognitive load and have dramatic results on problem success \cite{leinonen2021exploring, bouvier2016novice}.  Feedback also plays a critical role in learning~\cite{hattie2007power, vollmeyer2005surprising}.  Drill and practice exercises should be accompanied by solutions that can be used for the provision of immediate feedback, which in turn can prompt reflection and promote self-regulated learning behaviours \cite{shute2008focus}.  The manual generation of suitable repositories for large-scale drill and practice places a significant burden on instructors.


\subsection{Scalable problem generation}

A number of approaches have been explored for the automated generation of questions that could be used for drill and practice exercises.  These approaches commonly involve the use of question templates \cite{Zavala2018semantic, liu2018large} or parameterized questions \cite{Hsiao2009adaptive}.  In such cases, experts carefully design templates with selected elements that can be randomly generated or drawn from a pool of candidates.  Although such approaches can be used to generate a large number of questions, there remains significant human effort in constructing the templates and challenges in generating questions of equivalent difficulty when that is required \cite{denny2019fairness}.  

\subsubsection{Programming problems in computing education}
In certain domains, such as computing education, novel approaches have been employed to generate certain classes of problem. For example, Thomas et al. describe the use of a stochastic tree-based generation algorithm for producing program-tracing practice questions \cite{thomas2019stochastic}.  The approach was effective at generating multiple-choice questions with effective distractors, however was limited to producing a fairly narrow range of problems.  Similarly, Fowler and Zilles describe a novel approach for producing large pools of \emph{programming questions} through a permutation strategy \cite{fowler2021superficial}.  They identified a set of eight superficial problem description surface features that could be modified without significantly impacting the structure of the problem's solution code.  These surface feature permutations include changing the names of arguments to a function, or reversing the polarity of a question (for example, changing a question that works with positive numbers to one that works with negative numbers).  Starting with a base question, these permutations are then applied to produce eight novel variations of the problem.  One of the motivations for this work was to prevent students memorising questions and their answers when used on high-stakes exams.  Although the approach appeared promising for reducing this behaviour in students, generating good base questions requires manual human effort, and the number of permutations possible per base question is fixed.  The generation of programming questions, in particular, poses a difficult challenge in computing education.  There are usually many correct solutions to a programming problem, and so an instructor must define a comprehensive suite of test cases to dynamically verify potential solutions.  Lobb and Harlow describe an automated assessment tool for delivering drill and practice programming problems and note this as a key limitation: ``it must be mentioned that writing good quiz questions and good tests can be very time consuming even for low-level programming courses'' \cite{lobb2016coderunner}.

\subsubsection{Word problems in mathematics education}

In mathematics education, the use of \emph{word problems} is ubiquitous and their use has been widely studied \cite{verschaffel2020word}.  Word problems are presented as a natural language description of a scenario in which numerical data embedded within the description must be identified and extracted for the application of appropriate arithmetic operations. Generating math word problems is of great interest and many template based solutions have been explored.  For example, using manually defined templates with rules \cite{polozov2015personalized} or using templates where nouns and verbs are replaced with appropriate words from the desired topic \cite{koncel2016theme}.  Although such approaches can be used to generate high quality questions, as with any template-based approach, significant manual effort is required to generate new domain-specific templates. 

Recently, neural network models have been proposed for generating and solving math word problems automatically
\cite{zhou2019towards, wu2022automatic, huang2018neural}.  For example, Zhou et al. explore a novel fusion mechanism to incorporate equation and topic information combined with an entity enforced loss approach \cite{zhou2019towards}.  Although their model outperformed several baselines models, when the generated problems were rated by humans they scored well for topic relevance but fairly neutrally for equation relevance.  Wu et al. explore a specific topic-expression co-attention mechanism to overcome the limitations of sequence-to-sequence neural network approaches, which include the generation of unsolvable problems or problems that are unrelated to the topic words and expressions \cite{wu2022automatic}.  Their model, fine-tuned via reinforcement learning, tended to generate more complete and solvable problems when compared to baseline models.  

Approaches such as these are very promising, yet the models are designed to take an underlying equation for the word problem as input.  A more general solution, which produces novel equations as well as novel natural language scenarios, would be of particular value for application to the problem of constructing comprehensive repositories of drill and practice problems. 

\subsubsection{Learnersourcing and crowdsourcing}

A very different approach to the generation of large drill and practice question banks involves leveraging the effort of many humans.  Crowdsourcing is the practice of having a large group of individuals each make a small contribution towards a common goal.  One of the most widely known examples of a crowdsourcing project is the free online encyclopedia, Wikipedia\footnote{https://en.wikipedia.org} in which volunteers write and edit articles.  There also exist paid crowdsourcing services, such as Amazon's Mechanical Turk\footnote{https://www.mturk.com}, in which problems are divided into small microtasks and solved by harnessing human computation.  

Learnersourcing is a unique type of crowdsourcing in which students work collaboratively to generate shared learning resources \cite{kim2015learnersourcing}.  In computing education, for example, learnersourcing has been used to create multiple choice questions~\cite{denny2008peerwise,khosravi2019ripple}, introductory programming assignments~\cite{denny2011codewrite,pirttinen2018crowdsourcing}, and SQL exercises~\cite{leinonen2020crowdsourcing}.    Although students can derive learning benefits from the generative activity of creating content, there are several challenges to its use for producing usable question banks.  One of the most widely cited issues with learnersourcing is the frequently low quality of the resources produced by non-experts \cite{abdi2021quality, yang2016student}.  In addition, poor motivation on the part of students can also be a reason why learnersourcing approaches fail to generate useful resources \cite{singh2021whats}.

\subsection{Large language models}

%\cite{cobbe2021training}

%\todo[inline]{these first three paragraphs are verbatim copys from icer paper. Needs rephrasing and less emphasis on code generation and maybe something about math}

Recently, there has been great progress on generative NLP methods such as OpenAI's GPT-3~\cite{brown2020language} that are capable of generating text that can be hard to distinguish from text written by humans~\cite{brown2020language}. These are deep learning models and their performance relies on both a vast number of parameters for the models (175 billion in the case of GPT-3) as well as an extensive corpus of text for training (570GB of text for GPT-3). Codex~\cite{chen2021evaluating}, also by OpenAI, is similar to GPT-3, but has been trained with a very large number of public source code repositories from GitHub. While GPT-3 is primarily used to create novel content based on existing content, the goal of Codex is to both translate natural language to source code and vice versa, and to generate/auto-complete source code from given source code. 

Both GPT-3 and Codex have been previously used to solve math and programming exercises respectively. For math word problems, Cobbe et al.~\cite{cobbe2021training} observed that while GPT-3 was relatively poor at solving primary school math problems, the performance could be improved by separately training verifiers that rank outputs from the large language model and using the best option as the solution. In the context of solving programming exercises, Finnie-Ansley et al.~\cite{finnie2022robots} observed that Codex was able to correctly answer most introductory programming problems and that when given typical introductory programming exam questions, Codex performed better than the average student.

% In addition to OpenAI's Codex, other generative machine learning models capable of generating natural language from source code and/or vice versa have been developed. One of the earliest such models is Microsoft's CodeBERT~\cite{feng2020codebert}. CodeBERT has been trained with natural language-programming language pairs and is capable of generating source code documentation automatically similar to Codex. Another recently presented model is DeepMind's AlphaCode~\cite{li2022competition}, which is capable of performing at the level of a median competitor when presented with competitive programming competition problem prompts.

In this work, continuing on our prior work~\cite{anonymized2022automatic}, we explore the potential of such models for generating drill and practice style problems.  By replacing the human effort in a crowdsourcing model with the computational effort of large language models, a very large quantity of content can be generated quickly.  Much like a typical learnersourcing approach, a human expert can view, evaluate and potentially adjust the generated artefacts.  In addition, this expert can also provide basic priming information, such as an example problem and desired contextual information.  We use the term robosourcing to describe this new approach.  % We present a prototype system that generates robosourced drill and practice exercises, and evaluate the tool in the context of two cases studies involving typical problems from mathematics and computing education.


% \todo[inline]{something extra for the examples below?}

% These recent models have multiple applications. One application that has been proposed is to help programmers fix insecure code. Pearce et al.~\cite{pearce2021can} analyzed the performance of Codex and similar models for repairing source code containing security flaws and found that through providing a carefully constructed prompt for the model, they were able to patch security issues in programs in some cases. Another study by Pearce et al.~\cite{pearce2022pop} analyzed the possibility of utilizing Codex for reverse engineering. In their study, they provided Codex decompiled code and prompted Codex to explain the purpose of the code. Their results indicated that while there is promise in utilizing models such as Codex for reverse engineering as Codex could correctly answer slightly over half of the questions authors asked it about code, the authors note that further development is required before Codex could readily be used for reverse engineering. One approach they propose is fine-tuning the model by providing it context-specific training data (in their case, decompiled source code).

% \subsubsection{Codex and code generation}

% The most common use case for Codex is generating new code from either a provided code fragment or from a natural language description of a problem.  GitHub Copilot, which is the editor plug-in that is powered by OpenAI Codex, promises to generate code suggestions ``for whole lines or entire functions right inside your editor''. Indeed, the tagline for Copilot is: ``your AI pair programmer".  A developer using this plug-in would typically receive real-time code suggestions as they are typing, or would explicitly provide a natural language description (for example, as a code comment) and then receive more comprehensive suggestions, such as entire functions, almost immediately.  In many cases, multiple suggestions are provided that the developer can simply cycle through and accept or reject. 

% This code-generation use case could be applied productively in several ways in computing education contexts.  For example, students could generate model solutions for historical assignment, test and exam problems, where solutions may not otherwise exist.  They could also generate alternative correct solutions for a problem they have solved, to reflect on their own solution and to compare different algorithms and language constructs.  As the accuracy of Codex improves over time, introductory computing pedagogy may shift away from low-level coding and towards problem decomposition and problem solving. 

% However, Codex is not limited to code-generation tasks, and can generate natural language output from code-based or prose-based input.  In the current paper, we explore how this capability can be used to support two novel use cases that relate to the programming exercise life-cycle (see Figure~\ref{fig:course-design}).  The first of these relates to the generation of programming exercises by the instructor.  Given an existing exercise as input, we explore whether Codex can generate novel variations of the exercise that could then be deployed to students.  The second of these relates to the generation of feedback to students.  Given source code as input, we explore whether Codex can produce useful natural language feedback on that code, particularly in terms of helping students detect bugs prior to submission for grading.  In general, the use of a tool like Codex to generate practice problems for computing students in various formats, and to provide useful feedback to students on their progress with those problems, offers great potential. 

% In the context of programming education, Finnie-Ansley et al.~\cite{finnie2022robots} studied the potential of Codex for solving introductory programming assignments. They found that Codex was able to correctly answer most introductory programming problems and that when given typical exam questions, Codex performed better than the average student. The authors note that considering the performance of Codex, and especially that the progress in this area has been rapid, there are clear consequences for introductory programming courses. For example, when models such as Codex that are capable of performing well on programming assignments become more and more common, it becomes increasingly easy for students to use these models to write code for them, essentially engaging in a new type of plagiarism. While Finnie-Ansley et al. focused mostly on potential challenges Codex-like models will introduce to introductory programming classrooms, our focus in this article is exploring potential opportunities these models can provide in that context.


% \subsection{Learnersourcing and crowdsourcing}

% Crowdsourcing is the practice of having a large group of individuals contribute towards a common goal. The common goal may be grandiose such as building the largest encyclopedia in the world (i.e. Wikipedia) or something more modest, such as coming up with ideas for improving the local neighborhood. Often, reaching the common goal can be divided into smaller tasks, such as writing a single entry into Wikipedia, which then contributes towards reaching the common goal. 

% While there exist paid crowdsourcing services, such as Amazon MTurk, researchers and educators have had students participate in crowdsourcing efforts. One such effort, commonly used in education, is to have students create assignments into assignment pools~\cite{denny2008peerwise,pirttinen2018crowdsourcing}, which then can be shared to other students for learning and rehearsal. This act of using students as a crowd in a crowdsourcing activity is sometimes referred to as learnersourcing~\cite{kim2015learnersourcing} -- in this article, we include learnersourcing to the more commonly used term \emph{crowdsourcing}. In computing education research, crowdsourcing has been used, for example, to create multiple choice questions~\cite{denny2008peerwise,khosravi2019ripple}, introductory programming assignments~\cite{denny2011codewrite,pirttinen2018crowdsourcing}, and SQL exercises~\cite{leinonen2020crowdsourcing}.

% \subsection{Generating practice problems}

% Drill and practice activities are popular in many educational contexts, and they are also highly effective.  In a review of the efficacy of commonly used learning strategies, Dunlosky rated "practice testing", particularly when
% repeated over multiple study sessions, as the most effective technique for enhancing learning and boosting student achievement \cite{dunlosky2013strengthening}.  The benefits of frequent practice testing are widely known and reported even in popular media outlets.  A 2011 article in the New York Times, entitled ``To Really Learn, Quit Studying and Take a Test''\footnote{https://www.nytimes.com/2011/01/21/science/21memory.html} espoused the unique benefits of being tested when compared with several other common study techniques.  The benefits of drill and practice activities are underpinned by the \emph{testing effect}, the robust phenomenon that being tested on previously studied material is more beneficial to long-term retention of the material than not taking the test or even re-studying the material \cite{Roediger_2013_RPT}. This effect is well established both in controlled laboratory environments and in the classroom.  A meta-review of the testing effect in classroom environments showed clear evidence that frequent testing yielded positive effects on both perceived and actual learning outcomes \cite{Bangert_1991_FCT}.



% \subsection{Math problems}

% Generating math problems is of great interest, and many template based solutions have been explored.  For example, using manually defined templates with rules \cite{polozov2015personalized} or using templates where nouns and verbs are replaced with appropriate words from the desired topic \cite{koncel2016theme}.  Although such approaches can generate high quality questions, manual effort is required to generate new domain-specific templates and the variety of generated problems is limited by the template. 

% Zhou et al. propose an approach for automatically generating math word problems  \cite{zhou2019towards}.  Although it outperformed other models, when the generated problems were rated by humans, they scored well for topic relevance but fairly neutrally for equation relevance. 
% Huang et al. apply a sequence-to-sequence model to solve math word problems \cite{huang2018neural}.

% \subsection{Computing education problems}

% Generating good practice questions is very time-consuming, even for low-level programming courses \cite{lobb2016coderunner}.

% \subsubsection{Parameterized programming exercises}
% \cite{mirzaei2019annotated} -- Recent studies of student problem-solving behavior have shown stable behavior patterns within student groups. In this work, we study patterns of student behavior in a richer self-organized practice context where student worked with a combination of problems to solve and worked examples to study. We model student behavior in the form of vectors of micro-patterns and examine student behavior stability in various ways via these vectors. To discover and examine global behavior patterns associated with groups of students, we cluster students according to their behavior patterns and evaluate these clusters in accordance with student performance. 

% \subsubsection{Surface permutations -- isomorphic questions}

% %% Have just copied abstracts below
% \cite{fowler2021superficial} --- Assessing student performance on programming questions is important for introductory computer science courses, both for student learning and for ensuring students demonstrate competence. Part of being a competent programmer includes the ability to transfer learning from solved to analogous problems. Additionally, particularly in computer-based and online assessment, mitigating cheating efforts is another important consideration. One way to mitigate cheating is by randomly selecting from large pools of equivalent questions. In order to produce large pools of questions quickly, we used a permutation strategy to rapidly make new question variants by altering existing questions' surface features. In this work, we present the results of our first set of surface feature permuted questions in an introductory Python course. We find surface feature permutations to be an effective way to produce questions of a similar difficulty to other new questions for students while mitigating potential cheating. However, we also see permutations expose potential student knowledge fragility and transfer concerns, as performance on permutations of homework questions is not strictly better than performance on questions that are entirely new on assessments.






% \subsection{Copy-pasted 1}


% Introductory programming courses around the world interleave theory and practice, providing students opportunities on learning how to write programs guided by exercise statements, automated assessment systems, and course staff. Courses and course assignments are typically written so that they are increasingly complex, gradually introducing new concepts, seek to avoid overwhelming students i.e.\@ seek to avoid cognitive overload~\cite{duran2021cognitive}. Such a design can be seen as scaffolding that supports students in their zone of proximal development~\cite{vygotsky1978mind}, that is, their area of skills and knowledge where they cannot yet succeed in on their own, but where they can succeed in with guidance. As a student learns, the student's zone of proximal development also changes.


% %\todo[inline]{deliberate practice}
% %\todo[inline]{grit}
% %\todo[inline]{self-efficacy}
% %\todo[inline]{expectancy-value theory}
% % \todo[inline]{mastery learning}


% The design of programming courses and course assignments often reflects ideas of deliberate practice~\cite{ericsson1993role}, which is a systematic and purposeful type of practice that focuses on improvement of performance in a specific task. Continuing deliberate practice is sustained with grit~\cite{duckworth2013true}, i.e.\@ passion and perseverance for long-term goals, even when pursuing those goals feels difficult. Motivation towards assignments is influenced by the design of assignments; while very easy assignments have a high expectancy for success, their utility value is low, and as per expectancy-value theory~\cite{rosenzweig2019expectancy}, students may have little motivation to work with them. Similarly, too difficult assignments with little utility value can also lead to lower motivation~\cite{rosenzweig2019expectancy}, in addition to their likely negative contribution towards self-efficacy due to students' lack of skills needed to complete them~\cite{bandura1977self}. One practice in teaching introductory programming courses that has sought to avoid the situation where students are given too complex programming assignments is the use of many small programming exercises which help developing mastery through regular practice~\cite{allen2018weekly,edwards2020syntax,vihavainen2011extreme}. As students have different backgrounds, different skills, and differently evolving zones of proximal development, each student would likely benefit from a tailored set of assignments, maybe even with contextual cues tuned to their own interests as prior work has suggested that students' familiarity with the context can potentially be helpful~\cite{leinonen2021exploring}. Such large programming exercise pools would be tedious to develop~\cite{wrenn2018who, lobb2016coderunner}, however.

% % Such tailored sets of assignments could also help realize mastery learning~\cite{bloom}. -- mastery learning wasn't really about assingment sets until its


% %\todo[inline]{metacognition}
% %\todo[inline]{feedback}

% In addition to creating programming assignments, teachers often design feedback opportunities to course assignments. One common approach for providing feedback in introductory programming courses is the use of automated assessment systems~\cite{ihantola2010review,ala2005survey}, which at the minimum provide feedback on the correctness of programming assignments submitted for evaluation. As feedback plays a considerable role in learning~\cite{hattie2007power}, in addition to influencing approaches to learning by simply being offered~\cite{vollmeyer2005surprising}, it should be given with care; feedback can both improve self-efficacy and decrease self-efficacy~\cite{hattie2007power}, depending on how it is given. In general, formative feedback -- feedback given as a part of the learning process -- is preferred over summative feedback, i.e. feedback given after the learning process~\cite{shute2008focus}. In particular, formative feedback can be used to aid self-regulated learning and metacognition, helping students in becoming better learners~\cite{shute2008focus}. 


% Classroom practices and the way how the programming instruction is organized also matters~\cite{vihavainen2014systematic}. In particular, feedback opportunities can be included into classroom and lab sessions. For example, both peer instruction~\cite{crouch2001peer} and pair programming~\cite{williams2000strengthening} create opportunities for reflection; in peer instruction, the reflection is partially guided by the teacher responsible for the peer instruction questions, while in pair programming, students interact and reflect on the program that is being worked on. When pair programming, students also learn to reason and explain about code. 


==> 30-robosourcing-system.tex <==

\section{Methodology}



\subsection{Robosourcing system \label{subsec:method-robosourcing}}

For the present work, we implemented a prototype robosourcing system that allows the creation of math and programming exercises. The generic flow of creating exercises is outlined in Figure~\ref{fig:robsys}; first, a human provides a \emph{priming exercise} that includes a problem statement, a sample solution, and any expected themes and concepts (for programming exercises, automated tests can also be included). Once the priming exercise has been provided, the system creates a pool of exercises for evaluation. This is followed by a filtering phase where the system first automatically filters generated exercises, after which a human can do additional filtering. The filtered exercises can then be added to an exercise database.

For the prototype system, we used the Davinci-2 model from OpenAI Codex~\cite{chen2021evaluating}. However, we note that the system is not model dependent, the underlying generative model can be switched by replacing the underlying API. The number of exercises that the system creates, model specific parameters such as temperature and token length, as well as the themes and concepts can be configured in the system.

Filtering of the exercises is domain-specific. In the present version, for mathematics exercises, we provide options for (1) filtering out exercises where the solutions that follow the infix notation do not add up, (2) and filtering out exercises where the numbers present in the problem statement are not present in the sample solution. 
For the programming exercises, we provide options for (1) filtering out exercises where the sample solution cannot be run, (2) where the test cases do not pass, and (3) the code coverage of the tests is under a configurable threshold. Presently, the expected programming language is Python.
Further, for both the mathematics exercises and programming exercises, there is an option to search the problem statement from Google to assess whether the problem is novel. We acknowledge that the present automatic filtering, when enabled, can also filter out relevant exercises; this is an area with significant room for methodological advances. 

\begin{figure}[ht!]
\centering
\includegraphics[width=0.9\textwidth]{images/NeurIPS-ROPE.drawio.pdf}
\caption{Overview of our ``RobSys'' Robosourcing system. In the system, a user provides a starting point for creating exercises, which the system then uses to create an exercise pool. The exercise pool is filtered initially by the system based on options given by the user, after which the user can also filter out exercises. The exercises that are not filtered out are added to an exercise database.\label{fig:robsys}}
\end{figure}

\subsection{Research questions}

We evaluate robosourcing and the prototype systems by creating mathematics and programming exercises. For mathematics, we focus on primary school level exercises, as they are often in focus in prior literature, while for programming exercises, due to the same reasons, we focus on university level introductory programming.

Our research questions for the present study are as follows.

\begin{enumerate}
    \item[{\bf RQ1}] Is robosourcing a feasible way of generating drill and practice exercises for primary school mathematics?
    \item[{\bf RQ2}] Is robosourcing a feasible way of generating drill and practice exercises for university level introductory programming?
\end{enumerate}


\subsection{Approach and evaluation\label{subsec:approach-and-evaluation}}


% For camera-ready, add ACE paper below

To answer RQ1 and RQ2, we used the robosourcing system to generate practice exercises for primary school mathematics and university level introductory programming. To prime the mathematics exercises, we used the math exercises presented in~\cite{koedinger2004real}, while to prime the programming exercises, we used a variant of the speeding problem presented in ~\cite{venables2009closer} and a currency converter program. The keywords and themes used to prime the exercises are outlined in Table~\ref{tbl:priming-keywords}.

\begin{table}[h!]
    \centering
    \caption{Keywords used for priming exercise generation. The concepts are placed in sets to reduce the number of possible combinations.}
    \small
    \begin{tabular}{l|p{2.9cm}|p{2.5cm}|p{1.8cm}|p{1.8cm}}
    \toprule
    themes & programming concept set 1 & programming concept set 2 & math concept set 1 & math concept set 2 \\
    \midrule
    \multirow{5}{8em}{
        hiking,
        fishing,
        relationships,
        football,
        music,
        health,
        ice hockey,
        books,
        cooking
    }
    & function,   & class,      & sum, & subtraction, \\
    & parameters, & list,       & multiplication & division \\
    & dictionary, & conditional & conditional & \\
    & arithmetics & & & \\
    & & & & \\
    \bottomrule
    \end{tabular}
    \label{tbl:priming-keywords}
\end{table}

We generated exercises using the two priming exercises in Appendix~\ref{appendix:creation-priming-exercises}, varying the themes and concepts. Using a total of nine themes and two domain-specific concept sets, we generated a total of $9 * 2 * 2 = 36$ different combinations of inputs (themes $*$ domain-specific concept sets $*$ exercise primings). In addition, we explored two temperatures ($0$ and $0.75$) and created two exercises for each parameter combination. In total, this led to a sample of $36 * 2 * 2 = 144$ exercises for both mathematics and programming, totalling 288 generated exercises. For evaluation, we picked a random sample of 60 exercises for mathematics and programming each. 

The evaluation of the robosourced exercises was conducted both qualitatively and quantitatively. We evaluated the sensibleness, novelty, topicality, readiness for use and topicality of the randomly sampled generated exercises. For \emph{sensibleness}, we inspect whether the problem statement contains a sensible and practical problem for students to solve. For \emph{novelty}, we use Google search to see if we can find the exercise or a similar one online. For \emph{readiness for use}, we evaluate the consistence of generated answers to problems, and evaluate also generated tests for programming exercises. Readiness for use was evaluated only if an exercise was deemed sensible. 
For \emph{topicality} of the exercises, we analyse whether the generated problem statement incorporates the provided theme and concepts. 

%\todo[inline]{Somewhere mention that non-sensical exercises were ignored when calculating whether answer matches description}

%before they are redy to be given for students to work on.
%noticeable adjustments, i.e. more than simple typofixes and minor code adjustments, to the programming exercises and the associated sample solution and tests. Further, when analyzing the programming exercises, we collected notes identifying common pitfalls and issues, which we summarize in the results.

The analysis was conducted by four researchers. Each researcher worked on a subsample of the exercises. The researchers assessed the focused items with \texttt{Yes} / \texttt{No} / \texttt{Maybe} statements, qualitative notes were also added. All the \texttt{Maybe} answers were then discussed by at least two researchers to determine the proper label (\texttt{Yes} or \texttt{No}). 

% \todo[inline]{jatka}

% outlined in Table~\ref{tab:exercise-rubric}
%\begin{table}[ht!]
%     \small
%     \caption{\todo{fix}Assessment rubric \label{tab:exercise-rubric}}
%     \centering
%     \begin{tabular}{p{2.5cm}|p{8cm}|p{1.8cm}}
%     \toprule
%     Aspect & Question & Options \\
%     \midrule
%     Sensibleness & Does the problem statement describe a sensible problem? & Yes / No / Maybe \\% Yes = it makes sense as an exercise / No = it does not make sense as an exercise.\\
%     Novelty & Are we unable to find the programming exercise via online search (Google) of the problem statement? & Yes / No / Maybe \\%Yes = we cannot find one / No, we found one \\
%     Readiness: problem and solution & Does the problem statement match the model solution / answer? & Yes / No / Maybe \\%Yes = the solution solver the problem / No = the solution solves a different problem \\
%     Topicality: context & Does the problem statement topic match the given context priming concept? & Yes / No / Maybe \\
%     \midrule
%     Topicality: function / class & Is the problem statement about a function or class when that concept is provided as priming concept? & Yes / No / Maybe\\
%     Topicality (programming): list / dictionary & Does the problem statement incorporate a list or a dictionary when that concept is provided as priming concept? & Yes / No / Maybe\\
%     \midrule
%     Topicality (math): sum+multiplication / subtraction+division & Does solving the problem require sum and multiplication or subtraction and division when those concepts are provided as priming concept? & Yes / No / Maybe\\
%     Free-form notes & Notes  & Free-form text \\
%     \bottomrule
%     \end{tabular}
% \end{table}

%\todo[inline]{Check maybes together (excluding concept present column, because there it means partially)}
%\todo[inline]{What about NAs?}
We computed the \texttt{Yes} / \texttt{No} answers to provide quantitative results. For the programming exercises (RQ2), we also explore three further questions related to the readiness of use of the exercises; 1) can the sample solutions could be run, 2) do the sample solution pass the automated tests, and 3) what is the statement coverage of the automated tests. These analyses were conducted programmatically\footnote{Analysis of statement coverage of automated tests was conducted using \texttt{Coverage.py} version $6.3.2$ (\url{https://coverage.readthedocs.io/})}. For the programmatical analysis we used the full set of 144 generated exercises instead of the random sample of 60 exercises used for the qualitative labelling.

% . These questions are outlined in Table \ref{tbl:programming-exercise-automated-rubric} and the answers to the questions were obtained programmatically;

% \begin{table}[ht!]
%     \small
%     \caption{Automated assessment rubric}
%     \label{tbl:programming-exercise-automated-rubric}
%     \centering
%     \begin{tabular}{p{4cm}|p{6cm}|p{4cm}}
%     \toprule
%     Aspect & Question & Answer\\
%     \midrule
%     Readiness: solution runnability & Can we run the sample solution without errors & Yes / No / NA\\%(Yes = the code runs without errors / No, attempting to run the code causes an error)? \\% automatically from running tests
%     Readiness: solution and tests & Does the sample solution pass the unit tests? & Yes / No / NA \\ %Yes = all tests pass / No = the tests fail \\ % automatically from running tests
%     Readiness: test Coverage & To what extent do the unit tests cover the model solution (statement coverage)? & Percentage value (0 to 100) / NA\\% automatically from running tests
%     \bottomrule
%     \end{tabular}
% \end{table}


==> 40-results.tex <==

\section{Results}

\subsection{Math exercises}

% Seeds from:
% https://www.tandfonline.com/doi/pdf/10.1207/s15327809jls1302_1


The statistics for sensibleness, novelty, and whether the answer matches the exercise description of the evaluated mathematics exercises are presented in Table~\ref{tab:math-exercise-results}.
Out of the evaluated exercises, 75.0\% were sensible, 96.7\% were novel\footnote{Note that by our definition of novelty, non-sensical problem statements are rather certainly classified as novel}, and 51.9\% we such that the answer matched the problem statement. In addition, 96.7\% of the exercises matched the priming theme, and 36.7\% of the exercises completely matched the priming math concepts (i.e. all math concepts were present in solution), while 91.7\% of the exercises had at least one of the math concepts present.

\newcolumntype{x}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}

% \todo[inline]{60 not enough (because of systematic bottom to top / top to bottom evaluation, some topic combinations are underrepresented or overrepresented)}
\begin{table}[ht!]
\begin{threeparttable}
    \centering
    \small
    \caption{Summary of the manually evaluated math exercises. }
    \begin{tabular}{ c c c x{1.2cm} x{1.7cm} x{2.5cm} x{2.5cm} }
         \toprule
         Exercises & Sensible & Novel & Answer matches exercise & Matches priming theme & Matches priming math concepts (all) & Matches priming math concept\newline(at least one) \\
         \midrule
         60 & 75.0\% & 96.7\% & 51.9\% & 96.7\% & 36.7\% & 91.7\% \\
         \bottomrule
    \end{tabular}
    \label{tab:math-exercise-results}
%    \begin{tablenotes}
    %   \item  We consider an exercise \emph{sensible} if the requirements are described clearly within a context that makes logical sense, \emph{novel} if the exercise description returns no valid matches when used as the input for a search using Google, and has an \emph{answer correct} if the generated answer is the correct answer to the problem (does not need to include equation).
    % \end{tablenotes}
\end{threeparttable}
\end{table}

When going over the notes, we observed that the majority of the exercises where the answer did not match the problem description, the problems were minor and could be easily fixed. As an example, one sample solution suggested that `3 * 6 + 2 * 3` would be `21`, while the correct answer would have been `24`. Similarly, another sample solution had the answer in minutes, while the problem statement requested for hours. Additionally, a considerable number of the exercises categorized as non-sensible had in general a nice idea but poor execution, e.g. missing a value for a variable needed in the answer; such exercises could still be used to facilitate exercise creation and ideation.

The following verbatim example showcases an exercise generated with OpenAI Codex. The priming problem statement used to generate the exercise was the donuts problem from~\cite{koedinger2004real} (in Appendix~\ref{appendix:creation-priming-exercises-math}), the theme was ``fishing'', and the concept set was ``subtraction'', ``division'', and ``decimal''. 

\begin{tcolorbox}
\begin{Verbatim}[fontsize=\fontsize{9pt}{9pt},breaklines]
At the end of the day,
a fishing boat with a crew of 4 catches 38 fish and divides them evenly among the crew.
After the captain gets her share, she puts the extra 2 fish in a cooler for use later in the trip.
How many fish does each crew member get?
--Answer--
(38 - 2) / 4 = 9
\end{Verbatim}
\end{tcolorbox}

In the above example, the created exercise did not account for the concept ``decimal''. In the evaluation, we concluded that the exercise was sensible, novel, had an answer that matched the exercise, had a matching theme, but only matched the priming math concepts partially.

\subsection{Programming exercises}


The statistics for sensibleness, novelty, and readiness of the evaluated programming exercises are presented in Table~\ref{tab:programming-exercise-results}. Out of the evaluated programming exercises, 70.0\% were sensible, 95.0\% were novel, and 77.3\% had a matching sample solution. In addition, 90.0\% of the exercises matched the priming theme, and 50.0\% of the exercises completely matched the priming programming concepts, while 98.3\% of the exercises had at least one of the programming concepts present. The most common reason for a programming exercise not being sensible was the problem statement asking for the calculation of some sort of a value that required another value that was not available (e.g. amount of tax but missing price). In terms of the programming concepts, arithmetics was relatively often missing despite the programs featuring a `+`-symbol; in these cases, `+` was used for concatenating strings. 

% case with programming exercises that were not sensible was that 
 
%The free-form notes
%-- which were not mandatory -- 
%mostly discussed issues which included existence of redundant information, missing information, missing or incorrect values in sample inputs and/or outputs (some of the problem statements featured sample inputs and outputs), discussed mismatches between the problem statement and a sample solution, and outlined reasons why the automated tests would not pass. % In addition, the notes highlighted surprisingly good problem statements, as well as problem statements that felt a bit forced even though they were logical.



% \todo[inline]{should we write a high-level analysis of the notes here?}

\newcolumntype{x}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\begin{table}[ht!]
    \centering
    \small
    \caption{Summary of the manually evaluated programming exercises.}
    \begin{tabular}{ c c c x{1.5cm} x{1.5cm} x{2.3cm} x{2.5cm} }
         \toprule
         Exercises & Sensible & Novel & Matches sample solution & Matches priming topic & Matches priming concepts (all) & Matches priming concept\newline(at least one)\\
         \midrule
         60 & 70.0\% & 95.0\% & 77.3\% & 90.0\% & 50.0\% & 98.3\% \\
         %Speeding check & 120 & 75.0\% & 81.8\% & 76.7\%  \\
         \bottomrule
    \end{tabular}
    \label{tab:programming-exercise-results}
\end{table}


The statistics for the programmatic analysis that was conducted on all of the 144 created programming exercises are presented in Table~\ref{tab:dynamic_analysis_results}. Out of the 144 programming exercises, 136\footnote{\label{fn:autoextraction-imperfect}The actual count is slightly higher, since this value is computed from programmatically extractable content (requires the relevant keyword wrapped with double dashes ``--'' from priming in the generated content).} had a sample solution (94.0\%). From the 136 sample solutions, 133 (97.8\%) could be executed (i.e. running the code did not produce any errors). A total of 135\footref{fn:autoextraction-imperfect} programming exercises had automated tests. From the 135 programming exercises with tests, 85 had a sample solution that passed the automated tests. Out of the 85 programming exercises with a sample solution and passing automated tests, 83 had a 100\% statement coverage, and the statement coverage averaged over all the 85 programming exercises was 99.3\%. 

When inspecting the exercises with automated tests that did not pass, the most common issue was a flaw in calculations. As an example, one test expected that `10 / 1' -- after replacing variables with their values -- was equal to `2.8', while another -- again after replacing variables with their values -- expected that `12 * 2` was equal to `30'. Fixing these manually would often be trivial.

%we observed that the most common issue was not related to the code logic, but in how the outputs were handled. In those cases, the sample solution printed a value, while the automated tests expected that the sample solution would return a value (e.g. the tests called a function and expected that the function would return a value, but the function printed a value). In addition, a common issue was that the tests expected specific numbers that were not possible with the inputs (e.g. checking whether a program correctly extracted and returned a list of even values from a list received as a parameter, a test provided the list \texttt{[1, 2, 3]} as an input to the function and expected that the function would return the list \texttt{[2, 4]}).


%\todo[inline]{rewrite (table is updated)}
% In the programmatic analysis results on readiness, presented in Table \ref{tab:dynamic_analysis_results}, we see that around 98\% of the time the generated sample solutions are valid runnable code, tests are generated and auto-extractable roughly 94\% of the time, while around 63\% percent of the generated solution pass the tests (this requires both a sound solution and sound tests).
% Surprisingly enough, when we have passing generated tests on average we got around 99\% test coverage. Further, we noted that in multiple cases only minor tweaks would have been necessary to transform failing tests into passing ones. And for the cases where tests were missing, we could simply add the generated exercise to the initial priming and the tests would likely be generated on a ``second'' run (yes, we tested this out).
%We computed the number of duplicates (exact matches) in the generated exercises and got a total of 9. All of the duplicates were generated with temperature setting $0$ that set the determinism of the generations to maximum. The higher temperature setting of $0.75$ produced no duplicates.

%  and 48 out the 51 passing test sets covered 100\% of the sample solution statements

%\todo[inline]{add discussion on duplicates -- from Wikipedia "An internal GitHub study found that approximately 0.1\% of generated code contained direct copies from the training data. One specific example has been raised, in which the model outputted the original code of the fast inverse square root algorithm, including comments and an incorrect copyright notice"}

\begin{table}[ht!]
\begin{threeparttable}
    
    \centering
    \small
    \caption{Summary of programmatic analysis of generated programming exercises}
    \begin{tabular}{c|cx{2cm}cccc}
         \toprule
                     & Has sample solution?  & Can run sample solution?  & Has tests?  & All tests pass?  & Test coverage\footnotemark[1] \\
        \midrule
         Percentages & 94.0\%                & 97.8\%                            & 93.8\%      & 63.0\%           & 99.3\%       \\
         n out of N  & 136 / 144             & 133 / 136                         & 135 / 144       & 85 / 135            & 83 / 85  \\
         \bottomrule

    \end{tabular}
    \begin{tablenotes}
         \item \footnotesize{$^1$The percentage is the mean of all computable coverages. The n out of N is counted as the number of full coverage (100\%) of number of all tests that did not fail (coverage can be computed).}
    \end{tablenotes}
    \label{tab:dynamic_analysis_results}
\end{threeparttable}
\end{table}

%\begin{tcolorbox}
%\small
%\begin{verbatim}
%Write a function called fishing, which takes in one parameter:
%a dictionary of fish, for example {"cod": 10, "salmon": 20, "tuna": 5}.
%The function should return a string in the following format:
%"You caught 10 cod, 20 salmon, 5 tuna. Total: 35 fish."

%--Sample solution--
%def fishing(fish_dict):
%  text = "You caught "
%  for key, value in fish_dict.items():
%      text += str(value) + " " + key + ", "
%  text = text[:-2]
%  text += ". Total: " + str(sum(fish_dict.values())) + " fish."
%  return text
%--Tests--
%class TestFishing(unittest.TestCase):
%  def test_fishing(self):
%    self.assertEquals(fishing({"cod": 10, "salmon": 20, "tuna": 5}), 
%    "You caught 10 cod, 20 salmon, 5 tuna. Total: 35 fish.")
%    self.assertEquals(fishing({"cod": 0, "salmon": 20, "tuna": 5}), 
%    "You caught 0 cod, 20 salmon, 5 tuna. Total: 25 fish.")
%    self.assertEquals(fishing({"cod": 0, "salmon": 0, "tuna": 0}), 
%    "You caught 0 cod, 0 salmon, 0 tuna. Total: 0 fish.")
%    self.assertEquals(fishing({"cod": 10, "salmon": 0, "tuna": 5}), 
%    "You caught 10 cod, 0 salmon, 5 tuna. Total: 15 fish.")
%    self.assertEquals(fishing({"cod": 10, "salmon": 20, "tuna": 0}), 
%    "You caught 10 cod, 20 salmon, 0 tuna. Total: 30 fish.")
%\end{verbatim}
%\end{tcolorbox}

Below, we show a verbatim example of a well formed programming exercise generated by OpenAI Codex that received a positive score on all our manual and automated evaluation criteria. It is generated using the ``speeding'' priming example exercise (in Appendix~\ref{appendix:creation-priming-exercises}), theme ``music'', and concept set of ``class'', ``list'' and ``conditional''.

\begin{tcolorbox}
\begin{Verbatim}[fontsize=\fontsize{9pt}{9pt},breaklines]
Assume that you are building a music library app. Create a class called MusicLibrary.
This class should have a constructor that takes in a list of dictionaries,
each of which has keys "name" and "artist". The constructor should create a
property called library that stores the list of dictionaries.
The class must also have a method called search that takes in the name of a song,
and returns the artist who sings it. If the song does not exist in the library,
the method should return None. The classes should also have a method called
get_artist_songs that takes in an artist name, and returns a list of songs from
the library by that artist.
--Sample solution--
class MusicLibrary:
  def __init__(self, songs):
    self.library = songs
  def search(self, name):
    for song in self.library:
      if song['name'] == name:
        return song['artist']
    return None
  def get_artist_songs(self, artist):
    songs = []
    for song in self.library:
      if song['artist'] == artist:
        songs.append(song['name'])
    return songs
--Tests--
class Test(unittest.TestCase):
  def test_library(self):
    songs = [{'name': 'Rude', 'artist': 'Magician'}, {'name': 'Sugar', 'artist': 'Maroon 5'}]
    library = MusicLibrary(songs)
    self.assertEquals(library.search('Rude'), 'Magician')
    self.assertEquals(library.search('Sugar'), 'Maroon 5')
    self.assertEquals(library.search('Love Yourself'), None)
    self.assertEquals(library.get_artist_songs('Magician'), ['Rude'])
    self.assertEquals(library.get_artist_songs('Maroon 5'), ['Sugar'])
\end{Verbatim}
\end{tcolorbox}

==> 50-discussion.tex <==

\section{Discussion and conclusions}

\subsection{Feasibility of robosourcing}

The results demonstrate that robosourcing is indeed a feasible approach for generating drill and practice exercises. To summarize our results, and our answers to the Research Questions 1 and 2, we observed that approximately one half of the robosourced math exercises and approximately one third of the programming exercises would be directly usable for teaching. 

The robosourced exercises were predominantly novel as they could not be found via Google search, and users can adjust the themes and domain-specific concepts that influence the output of the robosourcing process. 
This shows that LLMs such as OpenAI Codex, can be used to robosource a diverse and large pool of exercises that could even be targeted based on learners' interests. This is similar to prior work by Wu et al.~\cite{wu2022automatic} for generating math exercises: the main differences in our work is that the we use a generic\footnote{Codex is somewhat generic, although it is optimized for programming code.} LLM-based content creation system, while Wu et al. propose a new model specific for the task and also the Wu et al.'s model requires a teacher given equation to create a new worded problem. With our model teacher does not need to provide the underlying equation involved in the exercise but can create new equations.
The possibility for learners themselves to influence the content could also be a pedagogically apt choice as it would involve the learner more in the process, potentially also increasing motivation -- assuming the exercise quality is high enough to (mostly) not require manual evaluation.

%Further, given that generated exercise or automated filtering quality is high enough to not require expert evaluation, learners may themselves be given an option to influence the exercises they are given by allowing learner to robosource their own exercises with their preferred themes -- a potential motivating factor (active learning theory).

%\todo[inline]{somewhere, mention that could also provide just an equation for creating math problems, comparison to \cite{wu2022automatic} and something else?}

%\todo[inline]{small comparison to our old paper - newer codex model > older model - math stuff - robosourcing system}
 
%\todo[inline]{note, really, that robosourcing also created automatic tests -- !!!}


\subsection{Ethical considerations}
\label{subsec:discu-ethical}

Robosourcing systems can be used to make the process of creating exercises faster. While ideally this will give teachers more time for e.g. face-to-face support to students, it is possible that if such systems become common, fewer teachers are needed. This in turn could result in fewer employment opportunities for teachers. However, we see the human-in-the-loop aspect of these systems important and hope they are used to complement teaching and not to replace teachers.

Prior work on LLMs has found that they can contain biases, for example, towards minorities~\cite{solaiman2021process,xu2021detoxifying}. This could negatively impact the content of the robosourced exercises. Indeed, we did observe that the exercises created by these systems did seem to more commonly involve men in problem descriptions. However, we did not observe any offensive content. A similar concern is that LLMs might leak personally identifiable information present in the training data~\cite{carlini2021extracting}. We did not observe any such data in our evaluation.

%\todo[inline]{mentions potential to create offensive content and leak of personally identifiable information and that we found no such data}

Prior work related to LLMs and programming education has found that LLMs can be used to solve introductory programming exercises~\cite{finnie2022robots}. Thus, familiarizing students with these systems could increase plagiarism -- and it is potentially even more likely that exercises created by LLMs can be solved by LLMs compared to exercises created by teachers. One potential way to partly tackle this problem would be to use canary exercises. We observed that there are exercises where the sample solutions are incorrect -- these exercises could be used to try catch those engaging in plagiarism utilizing LLMs.

%- potential negative societal impacts
%- opettajien ja kustantajien työ potentiaalinen negatiivinen impakti
%- content against certain minorities; cite previous works on openai codex (black box), unclear of existing biases (e.g. dalle-biakset)
%  - example exercises seemed to more often involve men %as the examples (e.g. Mr. Jordan when using a basketball related exercise for priming)

% - nää large language modelit myös toisaalta mahdollistaa huijauksen opiskelijoiden taholta; jos tehtävä ja answer luotu näillä, niin todnäk myös opiskelija voi saada vastauksen näihin käyttämällä näitä tooleja
%   - tähän toisaalta se, että löydettiin myös tehtäviä joissa vastaus väärin, näitä voisi käyttää esim. canaryinä huomaamaan huijaavia opiskelijoita
%   -- codex ei tosin vedä 100\% samoja samoja vastauksia, joten toimii vaan karkeena heuristiikkana
% - autogenerated exercises that are not easily solvable by LLMs. 
% -- test picking generated exercises where answers are wrong?

% https://nips.cc/public/EthicsGuidelines

\subsection{Limitations of work}
\label{subsec:discu-limitations}

The main limitation of our work is that our evaluation was relatively small-scale. It is possible that with thousands of exercises, the content would start to repeat itself, which would decrease the utility of robosourcing. At the same time, as the robosourcing process is primed by a human, there is certainly room for variation. In addition, our evaluation was not an in-classroom evaluation, so we cannot presently state how pupils or students would react to the exercises. The present evaluation was conducted by the authors, who are both teachers and researchers with significant experience from teaching both primary school mathematics and university-level introductory programming.

We have used OpenAI Codex in our work, which is at the time of writing in private beta and thus not openly accessible. In the future, it is likely that using Codex (or a similar system) will incur a fee, which makes it harder for e.g. researchers from developing countries to replicate this work. Furthermore, we only evaluated a few potential configurations for the options for OpenAI Codex (e.g. temperature value, which controls randomness).

Lastly, we used Google Search for checking the novelty of the generated exercises. It is possible that all potential sources of data are not possible to be found by Google Search.

%\todo[inline]{used Google Search for checking novelty; it is possible all potential sources of data is not possible to find on Google; although students could not find these either (but could accidentally plagiarize exercises)}



% - sufficient evaluation?
% - have not done a big evaluation -- e.g. it's possible that with thousands of exercises, there would be more duplicates
% -- we don't know what would be a e.g. good temperature setting for quality exercises without much duplicates
% - have not done a in-classroom evaluation -- just an evaluation of the prototype by the authors (who are both  teachers and researchers)


\subsection{Future work}

While our results suggest robosourcing is feasible already, future work that improves LLMs performance will likely also lead to improved performance when these models are used for robosourcing. For example, newer LLMs such as Gopher~\cite{rae2021scaling} by DeepMind outperform GPT-3 (which Codex is based on). Similarly, we used Codex without any fine-tuning: future work should work on fine-tuning LLMs specifically for robosourcing, which is likely to lead to increased performance. Lastly, the LLMs used in robosourcing could themselves be improved by feedback from the human-in-the-loop evaluations, increasing their performance for the robosourcing task.

%\todo[inline]{improving LLMs based on the human-in-the-loop evaluations}

% - machine learning etc for improving filtering 
% of quality generated exercises
% - when LLMs improve, it is likely that the quality of robosourced exercises also improve similarly -- e.g. newer models by Google are better than GPT-3, so might be better for this task too
% - we used OpenAI Codex for programming and math exercises, which is tuned for source code -> results would likely improve if using fine-tuned models specifically for robosourcing (e.g. LLMs fine-tuned for generating math exercises)
% - autogenerated exercises that are not easily solvable by LLMs.

% - evaluation of created exercises by students in terms of learnersourcing

==> 60-conclusion.tex <==

\section{Conclusion}


ownership of content, creating 

\subsection{Future work}
- machine learning etc for improving filtering 
of quality generated exercises
